Quasiclassical electron transport in topological Weyl semimetals

Weyl fermions are powerful yet simple entities that connect geometry, topology, and physics. While their existence as fundamental particles is still uncertain, growing evidence shows they emerge as quasiparticles in special materials called Weyl semimetals (WSMs). These materials possess unique electronic properties and hold promise for future technologies. This thesis investigates how electrons behave in WSMs, focusing on the chiral anomaly (CA). The CA remains central in condensed matter physics, typically observed via longitudinal magnetoconductance (LMC) and the planar Hall effect (PHE). Although finite intervalley scattering can reverse the LMC sign, we identify another mechanism: a smooth cutoff in the linear dispersion, inherent to real Weyl materials, introduces nonlinearity that causes negative LMC even without intervalley scattering. Using a lattice model of tilted Weyl fermions and the Boltzmann approximation, we explore LMC and PHE, mapping phase diagrams in key parameter spaces. We also study the effects of strain, which acts as an axial magnetic field and influences diffusive transport. Our results show that strain-induced gauge fields can cause a strong LMC sign-reversal, unlike external fields which need intervalley scattering. The interplay of strain and external fields produces rich LMC behavior. We further predict distinct PHE responses due to strain. Finally, we extend the study to nonlinear transport, developing a theory for the chiral anomaly-induced nonlinear Hall effect (CNLHE). In Weyl semimetals, the nonlinear Hall conductivity shows nonmonotonic behavior and strong sign-reversal with scattering. In contrast, spin-orbit coupled metals show consistently negative, quadratic responses. We also explore pseudospin-1 fermions, finding enhanced sensitivity to internode scattering, revealing new transport signatures and broadening the scope of chiral anomaly studies.

==> app_ch1.tex <==
%\clearpage
%\addcontentsline{toc}{chapter}{Appendices}
\begin{appendices}
\chapter{\label{appendix}(Optional)}
\end{appendices}


\setcounter{equation}{0}
\setcounter{table}{0}
\setcounter{figure}{0}
%\baselineskip 24pt


    





==> app_ch4.tex <==
%\clearpage
%\addcontentsline{toc}{chapter}{Appendices}
\begin{appendices}
\chapter{\label{appendix_ch4}(Optional)}
\end{appendices}


\setcounter{equation}{0}
\setcounter{table}{0}
\setcounter{figure}{0}
%\baselineskip 24pt


    





==> app_ch6.tex <==
%\clearpage
%\addcontentsline{toc}{chapter}{Appendices}
\begin{appendices}
\chapter{\label{appendix_ch6}(Optional)}
\end{appendices}


\setcounter{equation}{0}
\setcounter{table}{0}
\setcounter{figure}{0}
%\baselineskip 24pt


    




